Reimagining GNN Explanations with ideas from Tabular Data

Explainability techniques for Graph Neural Networks still have a long way to go compared to explanations available for both neural and decision decision tree-based models trained on tabular data. Using a task that straddles both graphs and tabular data, namely Entity Matching, we comment on key aspects of explainability that are missing in GNN model explanations.

==> related_work.tex <==
\section{Related Work}

While we have presented three ideas from tabular data that could be adopted to GNN explanations, there are other ideas as well. We present them here as related work.

\cite{Doran2017WhatDE} mainly focused on three key notions of explainable AI across the research fields explored to this date namely - opaque systems, interpretable systems and comprehensible systems. It summarized the three notions with gentle insights into these stating that opaque systems were those where the mapping mechanism of the input features to the final predictions is completely invisible to the user. Interpretable systems were those where there existed a transparency in the models used so that the user understood how the inputs were mathematically mapped to get the outputs. It also shed light on the third notion i.e comprehensible systems which emitted symbols in so that the user utilized  these to relate the input features to the outputs.

\vspace{5mm}
\noindent
\cite{das2020opportunities} delved into XAI to provide interpretable explanations and further categorised XAI techniques based on \emph{scope, methodology and usage}. Model-agnostic post-hoc explainability was considered essential due to its integrative nature. Various perturbation and gradient-based models were explained under these categories, and the same was used to evaluate explanation maps. These models, when subjected to adversarial attacks, greatly affected feature importance and thus, might not help make a decision single-handedly.

\vspace{5mm}
\noindent
\cite{samek2017explainable} explored the uses of XAI beyond human-interpretability, i.e. detecting ﬂaws in the model and biases in the data. To explain the predictions of deep learning models, two approaches were used, namely \emph{sensitivity analysis} and \emph{layer-wise relevance propagation}. The methods were evaluated on three classification tasks, and it was concluded that LRP provided a more relevant explanation.

\vspace{5mm}
\noindent
\cite{Samek_2019} focused on the importance of transparency and explainability in AI. Various types of explanations and their respective information content and use in practice were explored. The intent of explainable methods and how one would want to use it was also interpreted. Subsequently, different methods to approach XAI (like surrogates and meta-explanations) were covered. Various approaches such as LRP, SA and SpRAy were suggested to evaluate explanations, and finally, the quality of evaluation was assessed.

\vspace{5mm}
\noindent
\cite{Yuan2020XGNNTM} proposed an approach to explain the black box nature of GNN’s using a method known as XGNN. A graph generator was used to produce graph patterns which aided in maximizing the accuracy of the final predictions. The graph generator was trained via a policy gradient method that used reinforcement learning on the information extracted from the training of the GNN. The method predicted the process of adding an edge to the generated graph. These were then trained on both synthetic and real world datasets. The results showed that XGNN explained the model-level interpretability of the GNN’s to some extent and also that these generated explanations could be used to further help improve the trained model.

\vspace{5mm}
\noindent
In \cite{elton2020self}, mutual information gives a measure of what we gain by modelling the random variables X,Y using the joint distribution P(X,Y) as opposed to modelling them using P(X)P(Y). Note that the latter is possible iff we assume that the RVs X and Y are independent. Hence to compute MI, we essentially have to estimate the PDFs P(X,Y), P(X), P(Y) which in general are intractable to estimate accurately. In general, for the problem mentioned in the paper, we are unlikely to have an analytical expression. And hence what ppl do in general is to obtain samples (X,Y) and fit distributions on top of it to obtain an approximations of P(X,Y), P(X), P(Y). And as the number of samples approaches infinity, there are some methods like Gibbs sampling etc. that guarantee that the approx. estimates P(X,Y), P(X), P(Y) converge to the true distributions.

\vspace{5mm}
\noindent
\cite{sun2019infograph} proposes InfoGraph based on maximizing mutual information between unsupervised graph representation learning and the representations learned by supervised methods.

\cite{huang2020graphlime} introduced GraphLIME, which as the name indicates is a version of LIME for Graph Neural Networks. They compared their solution GNN Explainer \cite{ying2019gnnexplainer} which follows a subgraph approach to explain predicted links.

%\cite{oberhofer2014beyond} presented a probabilistic matching engine to match entities in relational data. \cite{mudgal2018deep} presented a deep neural model for entity matching. \cite{qian2019systemer} proposed SystemER, an active learning based approach for entity resolution.
